Characterizing The Influence of Continuous Integration. Empirical Results from 250+ Open Source and Proprietary Projects

Continuous integration (CI) tools integrate code changes by automatically compiling, building, and executing test cases upon submission of code changes. Use of CI tools is getting increasingly popular, yet how proprietary projects reap the benefits of CI remains unknown. To investigate the influence of CI on software development, we analyze 150 open source software (OSS) projects, and 123 proprietary projects. For OSS projects, we observe the expected benefits after CI adoption, e.g., improvements in bug and issue resolution. However, for the proprietary projects, we cannot make similar observations. Our findings indicate that only adoption of CI might not be enough to the improve software development process. CI can be effective for software development if practitioners use CI's feedback mechanism efficiently, by applying the practice of making frequent commits. For our set of proprietary projects we observe practitioners commit less frequently, and hence not use CI effectively for obtaining feedback on the submitted code changes. Based on our findings we recommend industry practitioners to adopt the best practices of CI to reap the benefits of CI tools for example, making frequent commits.

==> garbage.tex <==
%%%%%%%% ABSTRACT 

%We recommend practitioners to (i) apply the CI best practices along with adoption of CI tools, (ii) consider their team's development context before adopting CI tools, and (iii) after adoption of CI, investigate if CI satisfies their needs by applying software analytics. 
%Therefore, we cannot claim that CI is the `silver bullet' for software development.  
%Why is this so? 

%In numerous occasions Agile practitioners have warned about the negative aspects of adopting Agile tools and techniques, without implementing the primary practices of Agile. They have coined this observation as \textit{``doing'' Agile, but not ``being'' Agile}. However such warnings are opinion-based, as Agile practitioners have provided little to no empirical evidence that supports their recommendations. We mine 150 open source software (OSS) and 123 proprietary projects to investigate if empirical evidence exists for the phenomenon: ``doing'' Agile, but not ``being'' Agile. In particular, we investigate if the Agile technique of continuous integration (CI) influences bug and issue resolution, as well as commit patterns. According to our empirical analysis, for OSS projects, we observe the expected benefits after CI adoption, i.e., more bugs are resolved, and more issues are resolved. However, for the proprietary projects, we cannot make similar observations. Furthermore, we observe proprietary projects to ``do'' Agile, but not ``be'' Agile, as these projects use CI tools, without implementing the primary Agile practices for example, making frequent commits. We recommend practitioners not to use Agile techniques such as CI, without adopting the necessary practices.    

%Use of CI tools is getting increasingly popular, yet how proprietary projects reap the benefits of CI remains unknown. To investigate the influence of CI on software development, we mine 150 open source software (OSS) projects, and 123 proprietary projects.   

%Why is this so? Our findings indicate that only adoption of CI might not be enough to improve software development. CI can be effective for software development if practitioners use CI's feedback mechanism efficiently, by applying the practice of making frequent commits. For proprietary projects we observe practitioners to commit less frequently, and hence not use CI effectively, for obtaining feedback on the submitted code changes. We refer to this observation as \textit{`doing' Agile, but not ``being'' Agile} which indicates practitioners' adoption of Agile tools such as CI, but not the core practices associated with Agile. We recommend practitioners to (i) apply the CI best practices along with adoption of CI tools, and (ii) consider their team's development context before adopting CI tools. 

%%%%%%%%% INTRODUCTION 
%In numerous blog posts~\cite{dobeagile:monica}~\cite{dobeagile:jim}~\cite{dobeagile:khan}~\cite{dobeagile:sahota}, Agile practitioners caution that some organizations pretend to ``do Agile'' without actually ``being Agile''; which implies the organization's use of Agile techniques and tools without actually adopting the necessary Agile practices. While their cautions seem sensible, the Agile practitioners do not provide any empirical evidence which demonstrates how well-founded these concerns are. Accordingly, this paper checks empirically for two observations:

%\begin{itemize}[leftmargin=*]
%\item{Are some projects ``doing'' Agile without ``being'' Agile?}
%\item{Do we observe any detrimental effects for projects that are ``doing'' Agile without ``being'' Agile?}
%\end{itemize}

%To investigate these two observations, we investigate the usage of continuous integration (CI), one of the primary techniques to implement agility for software projects~\cite{Beck:1999:XP}. 
% can be an expensive procedure. For example, the Travis CI license to support two concurrent jobs is 129 USD per month~\footnote{https://travis-ci.com/plans}

% our industry partner located at North Carolina, IBM, invested XXX dollars to implement CI tools for its software development projects

% our industry partner located at North Carolina, IBM, invested XXX dollars to implement CI tools for its software development projects
%state if proprietary projects can reap the benefits of CI, and provide clues that explain why or why not proprietary projects reap the benefits of CI.          

%In XXX IBM adopted CI tools for its proprietary projects. IBM's expectation was upon adoption of CI, the proprietary projects managed by IBM, would experience similar benefits as observant for OSS projects, with respect to bug resolution~\cite{vasilescu2015quality}, and issue resolution~\cite{Zhao:ASE17:CI}. One strategy to investigate if adoption CI benefited IBM's proprietary projects is to conduct an empirical investigation. Such empirical investigation can be beneficial is two aspects:  

%Influence and adoption of CI has also gained interest amongst researchers. Hilton et al.~\cite{hilton:ase2016:ci} have investigated adoption rate of CI in OSS Github projects. Other researchers have investigated if CI influences commit patterns~\cite{Zhao:ASE17:CI}, and issue resolution~\cite{Zhao:ASE17:CI} for OSS Github projects. But, how does CI influence bug and issue resolution for proprietary projects? This paper compares the influence of adopting CI between OSS and proprietary projects by mining data from 150 OSS projects and 123 proprietary projects. We obtain this collection of 273 projects from a cloud-programming development environment hosted by our industrial partner. 

%Similar to prior work~\cite{vasilescu2015quality}~\cite{Zhao:ASE17:CI}, we focus on the influences of CI on bug resolution, issue resolution, and commit patterns. We also focus on collaboration, as use of CI, being one of the primary Extreme Programming (XP) techniques, is expected to benefit collaboration amongst team members~\cite{Sharp:2008:XP:colla}. 

%Adoption of CI for proprietary projects is non-trivial, as the adoption process requires significant investment in tooling and infrastructure~\cite{Debbiche2014:CI:Barrier}. Our industrial partner IBM, located at North Carolina, USA invested significant resources to adopt CI. The purpose of adopting CI was to improve their software development process with respect bug resolution, collaboration, and issue resolution
% as reported in prior work
% We conduct an empirical study to investigate if adoption of CI yielded the expected benefits for IBM's proprietary projects
% One strategy to investigate if our industrial partner's expectations were fulfilled, is to conduct an empirical study
% (ii) identify potential practices related to CI, which can be used to reap the benefits of CI;
%enabling better discussions between management and programmers about CI.

%Hence, based on our empirical findings, we advise:
%\begin{quote}
%{\em Do not use the \underline{tools} from another community without also adopting the \underline{practices} of that community.}
%\end{quote}

%\begin{figure*}
%\includegraphics[width=0.95\textwidth]{plots/CI-BG.pdf}
%\setlength\abovecaptionskip{-1pt}
%\setlength\belowcaptionskip{-1pt}
%\caption{An example work-flow of the continuous integration (CI) process.}
%\label{figure-ci-bg}
%\end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%% BACKGROUND 

% Humble and Farley~\cite{Humble:2010:CD} attributes the introduction of CI to Beck~\cite{Beck:1999:XP}.

%\subsection{``Doing'' Agile vs ``Being'' Agile}
%\label{bg:rel:doing:being}

%In numerous blog posts, practitioners have discussed the subtle differences between ``doing'' Agile and ``being'' Agile. ``Doing'' Agile implies a team's adoption of Agile tools and techniques such as daily scrums and CI, whereas, ``being'' Agile refers to the proper adoption of the agile practices such as frequently releasing software to end-users~\cite{dobeagile:monica}. As a hypothetical example, a team may adopt a CI tool as part of their daily work-flow, but if they release software infrequently, then that would imply that the team is ``doing'' Agile, and not ``being'' Agile. Some agile enthusiasts provides the following rule of thumb: ``doing'' Agile leads to 20\% added benefits, whereas, ``being'' Agile leads to 200\% added benefits~\cite{dobeagile:jim}. One of the co-authors of the Agile Manifesto~\cite{agile:manifesto} stresses the importance of ``being'' Agile and stated ``stop doing Agile and start being Agile''~\cite{dobeagile:jimh}. However, ``being'' Agile is non-trivial, as suggested by an Agile practitioner who stated ``doing Agile can be achieved over night, being Agile is a journey.''~\cite{dobeagile:khan}. 

%In popular programming literature we observe practitioners to discuss about ``doing'' vs. ``being'' Agile in details. However, we find little empirical evidence that supports/extends, the observation of ``doing'' Agile vs. ``being'' Agile. We use 273 projects to investigate the observation of ``doing'' Agile vs. ``being'' Agile by quantifying the influences of CI on bug/issue resolution, collaboration, and commit patterns. To the best of our knowledge, this is largest such study of it's kind.

%http://agilitrix.com/2016/04/doing-agile-vs-being-agile/
%http://agileknowhow.com/2017/02/06/doing-agile-vs-being-agile/
%http://www.disciplinedagiledelivery.com/agile-transformation-factors/

%Even though the concept of CI was introduced in 2006, initial usage of CI was not popular amongst practitioners~\cite{Deshpande2008:ci}. However, since 2011, with the advent of CI tools such as Travis CI~\cite{travis:ci}, usage of CI has increased in recent years~\cite{hilton:ase2016:ci}. CI is also considered to be a pre-requisite to implement continuous deployment~\cite{mika:highway:cd}.

%When a software team adopts CI, the team has to follow a set of practices~\cite{Duvall:ci2007}. According to the CI methodology all programmers has to check-in their code daily, which are integrated daily~\cite{Duvall:ci2007}. Unlike, traditional methodologies such as waterfall, in CI, programmers get instant feedback on their code via build results. To implement CI, the team must maintain its source code in a version control system (VCS), and integrate the VCS with the CI tool so that builds are triggered upon submission of each commit~\cite{Duvall:ci2007}. Figure~\ref{figure-ci-bg} provides an example on how a typical CI process works. Programmer make commits in a repository maintained by a VCS such as, GitHub, and these commits trigger CI jobs on a CI tool such as Travis CI which executes, builds, tests, and produces build results. These build results are provided to the programmers as a feedback either through e-mails, or phone alerts~\cite{Duvall:ci2007} on their submitted code changes. Based on the build results, programmers make necessary changes to their code, and repeats the CI process again.

%The above-mentioned description implies the practice of making frequent commits playing a pivotal role on how programmers are using CI for feedback. But do programmers change their commit patterns upon adoption of CI? We answer this question by mining 273 OSS and proprietary projects. 

%\subsubsection{\textbf{Adoption}} Hilton et al.~\cite{hilton:ase2016:ci} mined OSS projects hosted on Github. They observed that most popular projects use CI, and reported that the median time of CI adoption is one year. They also advocated for wide-spread adoption of CI, as CI correlates with several positive outcomes. However, adoption of CI is non-trivial as suggested by other prior work; for example, Olsson et al.~\cite{olsson:stairway:2012} who identified lack of automated testing frameworks as a key barrier to transition from a traditional software process to a CI-based software process. Also, Hilton et al.~\cite{Hilton:fse2017:ci} surveyed industrial practitioners and identified three trade-offs to adopt CI: assurance, flexibility, and security. Rahman et al.~\cite{Rahman:RCOSE17} observed that adoption of CI is not wide-spread amongst practitioners. They investigated which diffusion of innovation (DOI) factors influence adoption of CI tools, and reported four factors: relative advantages, compatibility, complexity, and education. 

%The above-mentioned studies indicate that adoption of CI involves overcoming certain barriers, and adopting certain practices. Findings from these papers also highlight the importance of assessing if after adoption of CI, do software teams enjoy benefits such as increased collaboration, better bug resolution, and better issue resolution?

%\subsubsection{\textbf{Usage}} 
% Zolfagharinia et al.~\cite{zolfa:msr2017:cpan} mined 30 million builds of the CPAN ecosystem's CI environment, and characterized the evolution of build systems.
% Rausch et al.~\cite{rausch:msr2017:ci} investigated build failures from 14 Java-based systems and characterized 14 error categories. They also observed that process metrics have relatively more influence on CI build failures.

%As stated before, we take motivation from prior work~\cite{hilton:ase2016:ci}~\cite{Zhao:ASE17:CI}~\cite{vasilescu2015quality} that have studied CI usage on OSS projects, and answer four research questions. We first describe how we filter the collected projects, then we answer the four research questions. We follow the Goal-Question-Metric (GQM) approach~\cite{gqm:original} to conduct our empirical analysis. The goal of our paper is to quantify the influences of CI on bug resolution, collaboration, and issue resolution, for both OSS and proprietary projects. To achieve this goal we answer four research questions as described in Sections~\ref{meth:rq1},~\ref{meth:rq2},~\ref{meth:rq3}, and~\ref{meth:rq4}. Each of the research questions are answered by metrics, as described in their respective section. We select the GQM approach as this approach has been successfully used to conduct empirical studies in software engineering~\cite{bird:gqm1}~\cite{zheng:gqm2}.      
% Example projects include: Javascript libraries such as `AngularJS'\footnote{https://github.com/angular/angular.js}, and programming languages such as `Scala'\footnote{https://github.com/scala/scala}.
%Our assumption is that by selecting these GitHub projects we can start with a representative set of OSS projects that enjoy popularity, and provide good examples of software development.    



%\begin{itemize}[leftmargin=*]
%\item{\textit{Collaboration}: Number of pulls requests are indicative of collaboration, and the project must have at least one pull request.}
%\item{\textit{Commits}: The project must contain more than 20 commits.}
%\item{\textit{Duration}:The project must contain software development activity of at least 50 weeks.}
%\item{\textit{Issues}:  The project must contain more than 10 issues.}
%\item{\textit{Contributors}: The project must have at least eight contributors.}
%\item{\textit{Releases}: The project must have at least one release.}
%\item{\textit{Software Development}:The project must only be a placeholder for software source code.}
%\end{itemize}
%\normalsize  %%% now go back to normalsized equation

%\item{\textit{Availability of Data (Before and After Adoption of CI)}: The project must have at least one month of software development activity data available before and after adoption of CI. Our assumption is that availability of at least one month of software development data, both before and after adoption of CI, can be sufficient to conduct analysis.}

%Similar to prior work~\cite{Bird:SNA2006}~\cite{Bhattacharya:ICSE2012:GAP}, we construct collaboration graphs using software project meta-data. From the constructed graph we extract in-degree. In-degree, corresponds to the count of edges that are incoming to a node.  

%As projects can vary in node count, and needs to be accounted for~\cite{Hong:ICSME2011}. Similar to Hong et al.~\cite{Hong:ICSME2011} and Bird et al.~\cite{Bird:SNA2006}, we normalize median in-degree by the count of nodes. We use Equation~\ref{equ:mid}, we normalize median in-degree.  
%Figure~\ref{fig:meth:graph1} presents the list of modified files $File1$ and $File2$, the lines that were modified, and the programmers who modified the files. Figure~\ref{fig:meth:graph2} presents the resulting collaboration graph constructed from the modification history. Figure~\ref{fig:meth:graph3} presents nodes, edges, and in-degree of each nodes, for the constructed graph.


%Similar to issues, as stated in ~Section~\ref{meth:rq1}, and bugs, as stated in Section~\ref{meth:rq2}, we compute $NMID$, for all projects, before and after adoption of CI. We apply statistical tests, described in Section~\ref{meth:stat}, to determine if CI has an influence on collaboration.

%%%%%%%%%%%%%%% RESULTS 

% The start year of these 1,108 OSS and 538 proprietary projects are presented in Figure~\ref{fig:res:raw:start:year}. We report how many of the projects were filtered out by the first filter, Filter-1, in Table~\ref{res:table:sanity1}. The projects that are discarded when the steps given in Table~\ref{res:table:sanity1} are applied sequentially, from top to bottom

% \begin{figure}
% \subfloat[]{
%  \includegraphics[width=0.24\textwidth]{plots/OSS_START_YEAR_ALL.pdf}
%  \label{fig:res:raw:oss}
% }
% \subfloat[]{
%  \includegraphics[width=0.24\textwidth]{plots/PROP_START_YEAR_ALL.pdf}
%  \label{fig:res:raw:pro}
% }
% \setlength\abovecaptionskip{-1pt}
% \setlength\belowcaptionskip{-1pt}
% \caption{Count of projects that started in each year. Figure~\ref{fig:res:raw:oss} presents the count of OSS projects. Figure~\ref{fig:res:raw:pro} presents the count of proprietary projects.} 
% \label{fig:res:raw:start:year} 
% \end{figure}

% \begin{figure}
% \setlength\belowcaptionskip{-2pt}
% \includegraphics[width=0.45\textwidth]{plots/MonthsToAdoptCI.pdf}
% \caption{Time to adopt CI. The median time to adopt a CI technology is respectively 12.5, and 7 months for OSS and proprietary projects. The difference in the two distributions is significant  ($p-value < 0.001$, Cliffs Delta=0.2). }
% \label{res:months2ci}
% \end{figure}

%\begin{table}
%\footnotesize
%\centering
%\setlength\abovecaptionskip{-1pt}
%\caption{Projects filtered for each sanity check of Filter-1.}
%\begin{tabular}{|l|r|r|}
%\hline
%Sanity check                             & OSS   & Proprietary  \\ 
%\hline
%Commits $> 20$                           & 96    & 68           \\
%Issues  $> 10$                           & 89    & 60           \\
%\# Contributors $>=8$                    & 67    & 47           \\
%S\/W development only                    & 51    & 9            \\ 
%Duration $>= 50$ weeks                   & 46    & 12           \\
%Releases \textgreater 0                  & 44    & 136          \\
%Collaboration (Pull requests $> 0$)      & 54    & 35           \\
%\hline
%Project count after filtering            & 661   & 171          \\ 
%\hline
%\end{tabular}
%\label{res:table:sanity1}
%\end{table}

%Data Availability (at least one month)     & 0    & 0           \\

%From Table~\ref{res:table:sanity1}, we observe that 59.6\% of the GitHub showcase projects pass the recommended sanity checks by researchers.
%The 447 projects filtered by applying Filter-1 further emphasizes the need to validate software project data mined from GitHub.

%By applying Filter-1 we obtain 661 OSS and 171 proprietary projects. From Figure~\ref{fig:res:raw:start:year} we observe that in 2014, majority of the proprietary projects started, and by selecting projects on or after the year 2014, we obtain a comparable set of OSS and proprietary projects. 

%Figure~\ref{fig:res:ncb:oss} presents the normalized count of closed bugs in OSS projects. Figure~\ref{fig:res:ncb:pro} presents the normalized count of closed bugs in proprietary projects.
%For proprietary projects, the influence of CI is non-significant for closed bug count. The median $NCB$ values are almost similar, before and after adoption of CI, as observed from Figure~\ref{fig:res:rq2} and Table~\ref{table:rq2}.    

%\vspace{1mm} %1mm vertical space
%%%Lesson-2 in a box 
%\fbox{\begin{minipage}{25em}
%\textbf{\textit{\underline{Lesson-2}: Unlike proprietary projects, significantly more bugs are resolved in OSS projects after adoption of CI. For proprietary projects the influence of CI on bug resolution is non-significant.}}
%\end{minipage}}
%\vspace{1mm} %1mm vertical space

%\begin{table}
%\centering
%\setlength\abovecaptionskip{-2pt}
%\caption{Influence of CI on Closed Bug Count ($NCB$)}
%\small{
%\begin{tabular}{ |c|c|c| } 
%\hline
%\textbf{Measure} & \textbf{OSS}    & \textbf{Prop.}           \\ 
%\hline
%Mean             & (A:0.1, B:0.0)  & (A:0.0, B:0.0)  \\ 
%p-value          & $< 0.001$       & 0.07            \\ 
%Cliffs           & 0.3             & 0.1             \\ 
%\hline
%\end{tabular}
%}
%\label{table:rq2}
%\end{table}


%\begin{table}
%\centering
%\setlength\abovecaptionskip{-2pt}
%\caption{Influence of CI on Closed Bug Count ($NCB$)}
%\footnotesize{
%\begin{tabular}{ |c|c|c| } 
%\hline
%\textbf{Measure} & \textbf{OSS}    & \textbf{Prop.}           \\ 
%\hline
%Median           & (A:0.15, B:0.03)  & (A:0.03, B:0.04)  \\ 
%$\Delta$         & +4.0              & \cellcolor{lightgray}-0.25  \\ 
%Mean            & (A:0.1, B:0.0)    & (A:0.0, B:0.0)  \\ 
%p-value          & $< 0.001$         & 0.9            \\ 
%Effect size      & 0.3               & 0.1             \\ 
%\hline
%\end{tabular}
%}
%\label{table:rq2}
%\end{table}

%\begin{table}
%\centering
%\setlength\abovecaptionskip{-2pt}
%\caption{Influence of CI on Closed Issues ($NCI$)}
%\small{
%\begin{tabular}{ |c|c|c| } 
%\hline
%\textbf{Measure} & \textbf{OSS [$\dag$]}    & \textbf{Prop.}           \\ 
%\hline
%Mean             & (A:0.3, B:0.1)  & (A:0.0, B:0.0)  \\ 
%p-value          & $< 0.001$       & 0.6       \\ 
%Cliffs           & 0.5             & 0.0             \\ 
%\hline
%\end{tabular} 
%}
%\label{table:rq1}
%\end{table}
%The time to adopt CI, and release frequency for OSS and proprietary projects is also different as shown in Figure~\ref{res:months2ci}. We observe that the median time to adopt CI is 1.7 times longer for OSS projects, compared to that of proprietary projects. For OSS projects the median time to adopt CI is 12.5 months, which is consistent with prior research: Hilton et al.~\cite{hilton:ase2016:ci} reported that for GitHub projects, the median time to adopt CI is 12 months. From Figure~\ref{res:oss:prop:rel:mon}, we observe average release per month to be significantly higher for OSS projects ($p-value < 0.001$, Cliffs Delta=0.9).  

% \begin{figure}
% \setlength\belowcaptionskip{-2pt}
% \includegraphics[width=0.35\textwidth]{plots/REL_PER_MON.pdf}
% \caption{Average release per month for projects. The median average releases per month is respectively 1.0, and 0.01 for OSS and proprietary projects.}
% \label{res:oss:prop:rel:mon}
% \end{figure}
%Even though the difference in commit size increases significantly, the effect size of the observed differences is smaller than that of commit counts. 
%Our commit size-related findings are consistent with Zhao et al.'s~\cite{Zhao:ASE17:CI} observations: they observed commit size to increase after adoption of CI. For proprietary projects we do not observe significant differences in commit size before and after adoption of CI.  
%\begin{table}
%\centering
%\setlength\abovecaptionskip{-2pt}
%\caption{Influence of CI on Commit Patterns}
%\footnotesize{
%\begin{tabular}{ |p{1.25cm}|p{1.25cm}|p{1.25cm}|p{1.25cm}|p{1.25cm}| } 
%\hline
%            & \textbf{Commit Count} &          & \textbf{Commit Size} &  \\ 
%\hline
%Measure     & OSS             & Prop.          & OSS                   & Prop. \\ 
%\hline
%Mean        & (A:3.5, B:2.1)  & (A:1.7, B:1.7) & (A:138.6, B:85.0)    & (A:57.9, B:173.4)     \\ 
%\hline
%p-value     & $< 0.001$       & 0.9            & 0.001                & 0.9    \\ 
%\hline
%Cliffs      & 0.3             & 0.1            & 0.2                  & 0.1   \\ 
%\hline
%\end{tabular}
%}
%\label{table:rq4}
%\end{table}

%\vspace{1mm} %1mm vertical space
%%%Lesson-5 in a box 
%\fbox{\begin{minipage}{25em}
%\textbf{\textit{\underline{Lesson-5}: For OSS projects, the size of commits significantly increase after adoption of CI. For proprietary projects, the difference in commit size before and after adoption of CI is non-significant.}}
%\end{minipage}}
%One possible explanation of this finding might be how CI is adopted in proprietary projects: the CI practices followed in the OSS domain might not be followed in the similar manner in the proprietary domain, which is leading to the differences in collaboration increase. 
% Based on effect size, we observe that the influence of CI is not as large as closed issues or closed bugs for OSS projects, as reported in Section~\ref{res:rq1} and Section~\ref{res:rq2}, respectively.
%\begin{table}
%\centering
%\setlength\abovecaptionskip{-2pt}
%\caption{Influence of CI on Collaboration}
%\small{
%\begin{tabular}{ |c|c|c| } 
%\hline
%Measure     & OSS           & Prop.                      \\ 
%\hline
%p-value     & $< 0.001$     & $< 0.001$                  \\ 
%Cliffs      & 0.2           & 0.2                        \\ 
%\hline
%\end{tabular}
%}
%\label{table:rq3}
%\end{table}
%Figure~\ref{fig:res:nci:oss} presents the normalized count of closed issues in OSS projects. Figure~\ref{fig:res:nci:pro} presents the normalized count of closed issues in proprietary projects.
% Zhao et al.~\cite{Zhao:ASE17:CI} reported that for OSS GitHub projects, number closed issues increases after adoption of CI. Our expectation is that for our set of OSS GitHub projects we will observe the same
% The `delta' measure is presented in the $\Delta$ row. These findings are also evident form the box-plots presented in Figure~\ref{fig:res:rq1}.
%We answer RQ2 by reporting how many bugs are closed before and after adoption of CI. We calculate $NCB$ using Equation~\ref{equ:ncb}. 
%Vasilescu et al.~\cite{vasilescu2015quality} reported that for OSS GitHub projects, code quality does not suffer after adoption of CI. For our set of OSS GitHub projects we expect to derive similar conclusions i.e. number of closed bugs will increase after adoption of CI. 
%%%%%%%%%%%% DISCUSSION 

%\textbf{On the Differences Between OSS and IBM Projects} As reported in prior work~\cite{Paulson:TSE2004}~\cite{Robinson:esem2010:prop:oss}, our empirical analysis also provides clues on the differences between OSS and proprietary projects, which we discuss below:

%\begin{itemize}[leftmargin=*]

%\item{On average, CI adoption rate is quicker for proprietary projects compared to OSS projects. One possible explanation can be related to co-adoption of CI and VCS i.e., when proprietary projects were transferred to Github, they also adopted CI, leading to an overall decreased adoption time. Another possible explanation can be related to CI's perceived benefits: teams might be biased to adopt CI tools because of it's perceived benefits.}

%\item{Findings from Table~\ref{res:table:sanity1} suggest that proprietary projects are less likely to release frequently. Of the 538 projects, 25.2\% of the projects do not pass the check `Releases $> 0$'. On the other hand, the number is lower for OSS projects: 3.9\% (44 of 1,108). On the other hand, majority of the OSS projects are working software constantly changing to satisfy end-user needs. }

%\item{Release frequency for OSS projects is significantly higher than that of proprietary projects. As CI is a primary practice of XP, we expected to see frequent releases for both: OSS and proprietary projects. But as suggested by Figure~\ref{res:oss:prop:rel:mon}, proprietary projects have a smaller release frequency than OSS projects. The observation that OSS projects tend to release frequently is unsurprising: Raymond~\cite{raymond:cathedral:bazaar} in his `Cathedral and the Bazaar' book mentioned the practice of frequent releases as ``a critical part of the Linux development model''. One possible explanation can be attributed to the nature of projects: these proprietary projects may be used internally within the organization, or the team, which are not delivered as software or services to the end-users.} 

%\end{itemize}

%\textbf{``Doing'' Agile vs ``Being'' Agile} We have observed proprietary projects to make infrequent commits, and make infrequent releases. Both these practices are antitheses of two recommended Agile practices: making frequent code changes to get rapid feedback~\cite{Duvall:ci2007}, and releasing working software frequently~\cite{agile:manifesto}. We refer to this observation as \textbf{``doing'' Agile, but not ``being'' Agile}, for proprietary projects, because of the following observation: even though an Agile tool (CI) is used, the practices of Agile are not being applied. From Section~\ref{results} we observe the benefits of CI not to be applicable for proprietary projects, providing some empirical evidence to the claims of Agile enthusiasts: being Agile is more beneficial than doing Agile~\cite{dobeagile:jim}~\cite{dobeagile:sahota}. Our findings also suggest that OSS projects are more likely to `do' and also `be' Agile.  
%Even for OSS projects, the influence of CI is more observable for issue resolution (larger effect size), than bug resolution. 

% Our findings suggest that CI might not have the same influence on all software development attributes. 
% and obtaining feedback for bug/issue resolution
%\textbf{Changing Perceptions on CI Adoption:} In software engineering, practitioners hold strong perceptions in certain topics, which are formed primarily from personal experiences and peer interactions~\cite{Devanbu:ICSE2016:Belief:Evidence}. Also, practitioners often follow the `diffusion of innovation' rule, which states that practitioners prefer to learn from other practitioners who have already adopted the tool of interest~\cite{akond:agile2015:cd}~\cite{rogers2010diffusion}. Our empirical study can be helpful to practitioners who hold certain perceptions about CI adoption. For example, by reading a success story of CI adoption for an OSS project, a practitioner might be convinced that CI adoption is a good choice for his/her team. The constructed perception can be checked and contrasted with empirical evidence. For CI adoption, learning from other practitioners can be a starting point, but practitioners also need to (i) consider their teams' development context, and (ii) systematically assess, to what extent other practitioners' experiences hold.  

%%%%% THREATS 

%\textbf{Detection of CI Usage}: We have adopted a heuristic-driven approach to detect use of CI in a project. We acknowledge that our heuristic is limited to the three CI tools, and we plan to improve our heuristics by exploring the possibility to add more CI tools. 

%\textbf{Detection of Bugs}: We have relied on issues for which a set of keywords appear to identify bugs. Even though keyword-based strategies have been used in prior work~\cite{emse16:zhang:dpm}, we acknowledge that a keyword-based strategy can be limiting. In future, we plan to apply manual analysis on the collected issues to determine which issues are actually related to defects.  
% We ask ourselves ``Can the results from proprietary projects be generalized to other proprietary projects?''. 

%\textbf{Methodology Choices}: Our approach is metrics-based, normalized by the time before and after adoption of CI, as well as by number of bugs and issues. Vasilescu et al.~\cite{vasilescu2015quality} used a `count of bugs per unit time' with a negative binomial regression model, to quantify the influence of CI on bug resolution. Zhao et al.~\cite{Zhao:ASE17:CI}, used regression continuity design, to quantify the influence of CI on issue resolution. Despite our methodology differences, our findings for OSS projects are consistent with Vasilescu et al.~\cite{vasilescu2015quality} and Zhao et al.~\cite{Zhao:ASE17:CI}'s findings. In future, we will explore other methodology choices to investigate the influence of CI on bug and issue resolution. 

% More gargage: 

%%We mine 150 OSS projects and 123 proprietary projects from a cloud-programming development environment hosted at Research Triangle, Raleigh, North Carolina, to answer the following research questions: 

%Hence, based on our evidence we observe CI does not significantly improve software development for proprietary projects. For proprietary projects, we also observe the practice of making frequent commits do not significantly increase after adoption of CI. For CI, making frequent commits is a recommended practice~\cite{Duvall:ci2007}. We conjecture that the benefits that OSS projects enjoy through CI adoption, are associated with the practice of making frequent commits. Commits provide a means for practitioners to get rapid feedback from CI tools on the submitted code changes. For proprietary projects, practitioners commit less frequently, implying they do not use CI effectively to get rapid feedback, which eventually may lead to lesser bug resolution, and issue resolution. The observed observations in proprietary projects can be termed as \textit{``doing'' agile, but not ``being'' agile}, which refers to teams' inclination of only adopting the tools and techniques of Agile, but not the core practices associated with it. 

%%We take motivation from these studies and investigate if adoption of CI is correlated with improvement of software development with respect to bug and issue resolution, and collaboration.    

%In Extreme Programming (XP), Continuous Integration (CI) is identified as one of the primary practices to implement agility for software projects~\cite{Beck:1999:XP}. CI systems integrate code changes by automatically compiling, building, and executing test cases upon submission of code changes. In recent years, usage of CI has become increasingly popular both for open source software (OSS) projects~\cite{hilton:ase2016:ci}~\cite{vasilescu2015quality}, as well as for proprietary projects~\cite{stahl:jss2017:ci:size}. Practitioners perceive adoption and usage of CI help them in catching bugs earlier, make integration of software changes easier, and make frequent releases of software product~\cite{fowler:ci:2006}~\cite{hilton:ase2016:ci}.

 

%Zhao et al.~\cite{Zhao:ASE17:CI} has reported that after adoption of CI, commit frequency and number of closed issues significantly increases. Will this observation generalize for proprietary projects? With respect to the development process, proprietary projects have fundamental differences with OSS projects~\cite{Paulson:TSE2004}~\cite{Robinson:esem2010:prop:oss}. To what extent CI influences bug and issue resolution for proprietary projects, as well as commit patterns requires systematic investigation. Through systematic investigation, we can determine if CI influences attributes of software development for OSS and proprietary projects in the same manner. 

%%Based on our findings we recommend practitioners to (i) consider team's development context before adopting CI tools, and (ii) after adoption of CI, investigate if CI satisfies their needs by applying software analytics. We warn practitioners from the proprietary domain not to expect CI to improve their software development process, only through CI tool adoption. We also recommend that CI can improve the software development process, if CI best practices are applied along with adoption of CI tools. 

%Continuous integration (CI) tools integrate code changes by automatically compiling, building, and executing test cases upon submission of code changes. 
%We recommend practitioners to prioritize their needs before adoption of CI.
%According to Hilton et al.~\cite{hilton:ase2016:ci}, OSS projects that use CI release twice as often than those who do not use CI.
%Therefore, we cannot claim that CI is the `silver bullet' for software development.  
%We observe collaboration to significantly increase after adoption of CI for OSS and proprietary projects.

%Adoption of CI can be prohibited by barriers, for example, practitioners can be skeptical about the benefits of CI, as they are unsure if the perceived benefits of CI will apply for their teams~\cite{Debbiche2014:CI:Barrier}. Other barriers to CI include, setting up and maintaining a CI server~\cite{Hilton:fse2017:ci}, and changing development and testing practices within the team~\cite{Debbiche2014:CI:Barrier}. If a team chooses to adopt CI, then the team has to overcome these challenges, which can cost the team additional resources, for example effort and time. With respect to CI adoption, practitioners can benefit from empirical case studies that address if adoption of CI significantly changes software development aspects such as collaboration amongst team members, resolution of bugs, and resolution of issues. These case studies can help practitioners to decide if CI is a good fit for their teams. Empirical evidence from the case studies, may also help address the skepticism that practitioners have about the benefits of CI adoption.  

%We investigate if adoption of CI influences software development attributes for both OSS and proprietary projects.

%In particular, we consider four attributes of software development: bug resolution, collaboration amongst team members, commit patterns, and issue resolution. 

%Recently, as more of the OSS tool suite is adopted by proprietary projects, we have become aware of large data sets where the influence of CI can be explored within proprietary projects. This raises an interesting research challenge: if we investigate proprietary software projects, will we find the same observations {\em outside} of the OSS software development process?
 
%Stahl et al.~\cite{stahl:jss2017:ci:size} surveyed practitioners and mined software data, and reported that continuity of continuous integration and organization size is correlated.  Stahl and Bosch~\cite{STAHL2014:JSS:CIPractice} identified CI practice differences by performing a systematic literature review, and proposed a descriptive model for the identified differences in practices. 

%Storm~\cite{storm:ci:saner2008} used the concept of backtracking to resolve build failures that happen in a CI system.

%\item{\textit{Git-based Development}: The project's development history must be completely available on Git. We exclude projects which have information hosted on other tools such as Subversion.}
%As our paper focuses on CI, we used another filter: `Filter-2:CI'. `Filter-2:CI' includes criteria that we use to identify which projects have sufficient information for analyzing the differences before and after CI adoption.

%opened (`Normalized Proportion of Open Issues' or $NOI$) and 
%`Proportion of Open Issues' ($OI$) and 
%We compute $OI$ and $CI$ respectively using Equation~\ref{equ:oi} and~\ref{equ:ci}. 
%\begin{equation}
%OI(p, m) = \frac{\text{total count of open issues in month $m$, for project $p$}}{\text{total count of issues in month $m$, for project $p$}}\label{equ:oi}
%\end{equation}

%\begin{equation}
%NOI (p) =  \dfrac{\sum_{i=1}^{M}OI(p, i)}{M}\label{equ:noi}
%\end{equation}

% To answer RQ2, we compute normalized open bugs (`Normalized Proportion of Open Bugs' or $NOB$) and closed (`Normalized Proportion of Closed Bugs' $NCB$).

%\begin{equation}
%OB(p, m) = \frac{\text{total count of open bugs in month $m$, for project $p$}}{\text{total count of bugs in month $m$, for project $p$}}\label{equ:ob}
%\end{equation}

%\begin{equation}
%NOB (p) =  \dfrac{\sum_{i=1}^{M}OB(p, i)}{M}\label{equ:nob}
%\end{equation}

%The above-mentioned methodology can tell us if CI influences commits patterns based on two metrics: commit frequency and commit size. However, to get a empirical on why CI has an influence on bug and issue resolution, we need to perform additional analysis. Our hypothesis is that if CI influences bug and issue resolution, and commit patterns then we will observe correlations between bug resolution and commit patterns, as well as between issue resolution and commit patterns. We use the Spearman correlation~\cite{spearman:reff} technique between the following pairs of values: ($NCC$, $NCB$), ($NCC$, $NCI$), ($NCS$, $NCB$), and ($NCS$, $NCI$). After adoption of CI we compare the correlation values for before and after adoption of CI. An increase in correlation value would indicate that if CI influences commits patterns, then such influence might be correlated with bug and issue resolution as well.         

%Similar to closed issues, we observe CI to have influence on closed bug count.
%Based on Cliffs Delta, unlike closed issue count, we observe the difference after and before adoption of CI to be medium

%We answer RQ4 by reporting the distribution of two metrics normalized commit count ($NCC$), and normalized commit size ($NCS$). 

%Based on Cliffs Delta, for OSS projects, the difference observed in commit count after adoption of CI is small. 

%\textbf{Correlation Between Commit Patterns With Bug and Issue Resolution}: Previously, in Section~\ref{meth:rq4} we have mentioned how we sued correlation analysis as a surrogate empirical method to explain if the influence of CI on bug and issue resolution can be explained by using the change in commit patterns due to influence of CI. We present the correlation values for OSS and proprietary projects respectively, in Tables~\ref{table:oss:corr} and~\ref{table:prop:corr}. The highlighted cell in grey indicates the p-value $< 0.05$, for the reported correlation co-efficient. From Table~\ref{table:oss:corr} we observe that our hypothesis holds for closed issues, as the correlation between $NCI$ and $NCC$ increase after adoption of CI, compared to that of before CI adoption. This finding suggests that the change in commit frequency due to CI is related to issue resolution, and can provide a potential clue on why more issues are resolved after adoption of CI. We also observe increase in correlation between commit sizes and closed issues, after adoption of CI. This finding suggests that after adoption of CI, programmers perform large-sized commits, which includes code changes to resolve necessary issues. Future research can investigate this explanation thoroughly.       

%According to Table~\ref{table:oss:corr}, the findings for bug resolution is opposite: we observe decreased correlation, after adoption of CI. Such finding provided opposite evidence to our hypothesis, and indicates that change in programmers' commit pattern behavior may not be related to bug resolution for OSS projects.  

%The influence of CI on commit count is also visible from Figure~\ref{fig:res:rq4}.

%\begin{table}
%\centering
%\setlength\abovecaptionskip{-2pt}
%\caption{OSS Projects: Correlation Between Commit Patterns With Bug and Issue Resolution}
%\footnotesize{
%\begin{tabular}{ |p{1cm}|p{1.25cm}|p{1.25cm}|p{1.25cm}|p{1.25cm}| } 
%\hline
%            & \textbf{Commit Count} ($NCC$) &          & \textbf{Commit Size} ($NCS$) &  \\ 
%\hline
%Measure     & Before CI             & After CI          & Before CI                   & After CI \\ 
%\hline
%$NCI$       & 0.06  & \cellcolor{lightgrey}0.18 & 0.03 & 0.13   \\ 
%$NCB$       & 0.05  & 0.02 & 0.01 & -0.06   \\ 
%\hline
%\end{tabular}
%}
%\label{table:oss:corr}
%\end{table}

%According to Table~\ref{table:prop:corr}, the correlation values between commit metrics ($NCC$ and $NCS$) and bug and issue resolution ($NCB$ and $NCI$), have decreased, after adoption of CI. This finding suggests that after adoption of CI, $NCI$ and $NCS$ decrease, as well as, $NCB$ and $NCI$.   

%\begin{table}
%\centering
%\setlength\abovecaptionskip{-2pt}
%\caption{Proprietary Projects: Correlation Between Commit Patterns With Bug and Issue Resolution}
%\footnotesize{
%\begin{tabular}{ |p{1cm}|p{1.25cm}|p{1.25cm}|p{1.25cm}|p{1.25cm}| } 
%\hline
%            & \textbf{Commit Count} ($NCC$) &          & \textbf{Commit Size} ($NCS$) &  \\ 
%\hline
%Measure     & Before CI             & After CI          & Before CI                   & After CI \\ 
%\hline
%$NCI$       & 0.02  & -0.07 & 0.12 & -0.07   \\ 
%$NCB$       & 0.02  & -0.12 & 0.12 & -0.08   \\ 
%\hline
%\end{tabular}
%}
%\label{table:prop:corr}
%\end{table}

%\item{Figure~\ref{fig:res:raw:start:year} states that most of the proprietary projects started on or after 2014, whereas, the start year for OSS projects is rather uniform from 2008 to 2017. One possible explanation can be the proprietary projects are previously hosted on a different VCS system such as Mercurial, later on, these projects were transferred to Github. This observation highlights how adoption and use of VCS systems such as Github can be different between OSS and proprietary projects, which needs to be accounted for.}
%Future research can investigate this explanation in details.
%\item{Findings from Table~\ref{res:table:sanity2} also hint that compared to proprietary projects, OSS projects are less inclined to adopt CI, as 67.7\% (448 of 661) projects do not use CI. The statistics are lower for proprietary projects 26.9\%(46 of 171). We advocate researchers to investigate this phenomenon in details.}

%Releasing software frequently to end-users is one of the principles of the Agile manifesto~\cite{agile:manifesto}. Even though an agile tool (CI) is being used in OSS and proprietary projects, we notice OSS projects to actually implement the agile principle

%\textbf{The `Cargo Cult' Phenomenon:} Above-mentioned discussion, and our findings presented in Section~\ref{res:rq4} hint an anti-pattern for proprietary projects: programmers of these projects are not implementing the practice of making frequent commits. One possible explanation of this anti-pattern can be attributed to how practitioners adopt a tool. Practitioners might be adopting CI tools, but not the best practices associated with CI adoption such as making frequent commits. Such behavior from practitioners can be attributed as the `cargo cult' phenomenon~\cite{Lindstrom93}; i.e. when a culture is adopted, but the essential practices of the culture is ignored. For proprietary projects, we see practitioners  treating CI as a cargo cult; i.e. they  adopt CI tools, but not the best practices of CI. Keeping this phenomenon into account, we recommend practitioners to apply the best practices of CI, along with CI tool adoption.

%Researchers~\cite{Spinellis07}~\cite{Brooks87} in prior work warned against `silver bullets' in software engineering. In Brooks' 1986 paper `No Silver Bullet-- Essence and Accident in Software Engineering'~\cite{Brooks87}, he warns against hyping a technology as the `silver bullet' that will automatically kill the werewolves which bedevil software engineering:

%\begin{quote}
%{\em ``There is no single development, in either technology or management technique, which by itself promises even one order of magnitude improvement within a decade in productivity, in reliability, in simplicity.''~\cite{Brooks87}}
%\end{quote}

%We recommend teams to adopt CI if CI satisfies their needs. Based on our findings, if a software team is developing an OSS project and emphasizes on issue resolution then CI might be a good fit for the team. As another example, if a software team emphasizes on collaboration, then adoption of CI can be a good decision because empirical evidence suggests that CI influences collaboration for both: OSS and proprietary projects. In summary, . We also recommend practitioners to continuously quantify the influence of CI on their needs, using software analytics.  

%\textbf{Data-driven Decision Making:} Based on our findings, we recommend software practitioners to mine features such as bug and commit metrics form version control meta-data, and use these features to make informed decisions. We also recommend practitioners to conduct software analytics in a continuous manner, instead of considering software analytics as a `one-time-thing'. Software development process, and requirements evolve over time, and by applying software analytics continuously, practitioners can make decisions based on the recent data. We have observed from Section~\ref{res:rq4} that programmers' commit patterns change after CI tools are adopted. Through continuous analytics, practitioners may understand which practices are changing within the team, at what time, and which tools are influencing that change. 

%\textbf{Introduction of CI}: CI can be introduced in the later phases of project, and that can bias our metric calculations and statistical analysis. We accounted for this bias by normalizing the metrics ($NCC$, $NCS$, $NCI$, $NBI$) with respect to time, measured in months.

%For OSS projects, similar to Zhao et al.~\cite{Zhao:ASE17:CI}, we observe number of closed issues to increase after CI. Similar to Vasilescu et al.~\cite{vasilescu2015quality} we observe number of closed bugs         

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%ICSE-SEIP-BACKGROUND-RELATED WORK%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%CI is also considered to be one of the fundamental pillars to implement DevOps, a relatively new software development methodology that advocates for the collaboration between the software development team and operations team~\cite{devops:ebert}~\cite{Humble:2010:CD}. 
%Deshpande and Riehle~\cite{Deshpande2008:ci} in their 2008 paper reported that OSS projects have not adopted the practice of CI. 
%In CI, the release cycle is short, compared to traditional methodologies.
%Debbiche et al.~\cite{Debbiche2014:CI:Barrier} interviewed practitioners from a Swedish telecommunication organization, and identified 23 adoption challenges related to CI.
%Shahin et al.~\cite{shahin:access2017:ci} investigated which practices should be considered while adopting CI, and provided four recommendations: reducing build and test time, increasing awareness on build results, supporting automated continuous testing, and defect detection.  
%However, their findings are limited to OSS projects. Whether or not their observations are generalizable for proprietary projects, introduces an interesting question. Such observation motivates us to perform an empirical study where we investigate usage of CI for both OSS and proprietary projects.

%\subsection{Silver Bullets and Cargo Cults}
%In software engineering, a
%        `silver bullet' refers to as a methodology or technology that improves an existing software development process, by fundamentally changing the software process of an organization~\cite{Brooks87}. Researchers~\cite{Spinellis07}~\cite{Brooks87} in prior work warned against `silver bullets' in software engineering. Brooks~\cite{Brooks87} warned against hyping a technology as the `silver bullet' that will automatically kill the werewolves which bedevil software engineering.
%        Similarly, we warn that adopting continuous integration is not a silver bullet that  dramatically improves  proprietary projects.

%\subsection{Cargo Cult}
%\label{bg:rel:cult}
        
%In anthropology,  a `cargo cult'
%is characterized by the adoption of a specific culture, while missing essential practices of that culture~\cite{Lindstrom93}. The name `cargo cult' derives from the belief which began among Melanesians since the 1900s where ritualistic acts such as, the building of an airplane runway will result in the appearance of  Western goods (i.e., `cargo'), via Western airplanes. We observe proprietary projects to adopt CI tools, but not implement a recommended best practice i.e. the practice of making frequent commits. We draw parallels between our observations for proprietary projects and the Melanesians: only adoption of CI tools is not enough to achieve the benefits of CI tools. The concern of this paper is that proprietary projects suffer from a `cargo cult' mentality with respect to CI tools.    


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%ICSE-SEIP METH%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

`Rust'\footnote{https://github.com/rust-lang/rust}, 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%ICSE-SEIP INTRO%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Is continuous integration (CI) useful? Adoption of CI has become increasingly common both for open source software (OSS) projects~\cite{hilton:ase2016:ci}, as well as for proprietary projects~\cite{stahl:jss2017:ci:size}. Prior research~\cite{vasilescu2015quality}~\cite{Zhao:ASE17:CI}~\cite{hilton:ase2016:ci} that have explored the influence of CI, have focused on OSS projects, and not for proprietary projects. Accordingly, in this paper, we ask ``is CI beneficial for proprietary projects?''.

To answer this question, we mine 661 OSS projects with 72,847 programmers from GitHub, and 171 proprietary projects with 6,620 programmers from our industrial partner at Research Triangle Park, North Carolina, USA. From that data, we suggest:
\begin{quote}
{\textit{\textbf{to reap the benefits of CI, do not just adopt CI
tools; it is also vital to adopt CI best practices.}}}
\end{quote}

To support this conclusion, we apply statistical analysis on the collected data, and answer the following research questions: 

\begin{description}[leftmargin=*]
\item{\textbf{\textit{RQ1: How does adoption of continuous integration influence issue resolution?}}} Significantly more issues are resolved after adoption of CI for OSS projects, but not for proprietary projects.

\item{\textbf{\textit{RQ2: How does adoption of continuous integration influence bug resolution?}}} Unlike proprietary projects, significantly more bugs are resolved after adoption of CI within OSS projects.

\item{\textbf{\textit{RQ3: How does adoption of continuous integration influence collaboration amongst team members?}}} After adopting CI, collaboration significantly increases for both, OSS and proprietary projects. The increase in collaboration is more observable for OSS projects, than proprietary projects. 

\item{\textbf{\textit{RQ4: Does adoption of continuous integration influence commit patterns?}}} Commit frequency and sizes significantly increases for OSS projects after CI adoption, but not for proprietary projects. 
\end{description}

%Hence, from our findings we observe that CI is not the `silver bullet' for proprietary software development, as CI does not significantly improve software development for proprietary projects.

Hence, based on our evidence we observe CI not to significantly improve software development for proprietary projects. The benefits that OSS projects enjoy through CI adoption, are associated with the practice of making frequent commits. Commits provide a means for practitioners to get rapid feedback from CI tools on the submitted code changes. For proprietary projects, practitioners commit less frequently, implying they do not use CI effectively to get rapid feedback, which eventually may lead to lesser bug resolution, and issue resolution. The observed phenomenon in proprietary projects can be termed as the `cargo cult phenomenon', where a team adopts a CI tool, but not the best practices associated with CI. 

The rest of this paper is organized as follows.
The next section discusses background and  related work. Our data analysis methodology is explained in Section~\ref{meth} which is followed by our findings in Section~\ref{results}. These findings are discussed in  Section~\ref{discussion}, followed by notes on the validity of our conclusions in Section~\ref{threats}.  

Before all that, we take care to stress the following point. There may well be benefits to CI that are not captured by the metrics we collect. For example, there  may be cultural benefits in introducing CI tools to an existing infrastructure. That said, we caution advocates of CI  not to hype their preferred approach. If users of CI technology were `sold' on that technology based on a promise that it will (e.g.) instantly increase bug resolution then, practitioners from proprietary projects may be dissatisfied with CI tools.


%Example of popular projects included in the GitHub showcase that we use for our analysis are: Javascript libraries such as `AngularJS'\footnote{https://github.com/angular/angular.js}, and`npm'\footnote{https://github.com/npm/npm}, and programming languages such as `Go'\footnote{https://github.com/golang/go}, `Rust'\footnote{https://github.com/rust-lang/rust}, and `Scala'\footnote{https://github.com/scala/scala}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\title{Continuous Integration: The Silver Bullet?}\subtitle{On The Merits of Continuous Integration for Proprietary Projects}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%% AUTHOR 

\author{Author1}
\affiliation{
  \institution{North Carolina State University}
  \city{Raleigh} 
  \state{North Carolina} 
  \postcode{27607}
}
\email{author1@ncsu.edu}

\author{Author2}
\affiliation{
  \institution{North Carolina State University}
  \city{Raleigh} 
  \state{North Carolina} 
  \postcode{27607}
}
\email{author2@ncsu.edu}

\author{Author3}
\affiliation{
  \institution{North Carolina State University}
  \city{Raleigh} 
  \state{North Carolina} 
  \postcode{27607}
}
\email{author3@ncsu.edu}

\author{Author4}
\affiliation{
  \institution{North Carolina State University}
  \city{Raleigh} 
  \state{North Carolina} 
  \postcode{27607}
}
\email{author4@ncsu.edu}


%%%%%%%%%%%%%%%%%%%%%%%%%% ABSTRACT 
% Continuous integration (CI) systems integrate code changes by automatically compiling, building, and executing test cases upon submission of code changes. Use of CI tools is getting increasingly popular, yet how CI influences the software development process for both, open source software (OSS) and proprietary projects remains unknown. Quantifying the influence of CI on software development process can help software practitioners make informed decisions on adoption and usage of CI. \textit{The goal of the paper is to help software practitioners in making informed decisions on continuous integration (CI) adoption and usage by mining open source and proprietary software repositories.} We investigate if CI influences four aspects of software development process namely, bug resolution, collaboration, commit patterns, and issue resolution. We 

%% Amongst the We observe that after adoption of CI, significantly more bugs and issues are resolved, and commits are more frequent for OSS projects. However, for proprietary projects, we do not observe any significant difference in bug resolution, commit patterns, and issue resolution. We conclude that CI is not the `silver bullet' for software development, as CI does not influence all studied aspects of software development for both: OSS and proprietary projects. Based on our findings we recommend practitioners to (i) consider team's development context before adopting CI tools, and (ii) after adoption of CI, investigate if CI satisfies their needs by applying software analytics.   

%%%%%%%%%%%%%%%%%%%%%%%%%%% INTRO
% Adoption of CI can be prohibited by barriers, for example, practitioners can be skeptical about the benefits of CI, as they are unsure if the perceived benefits of CI will apply for their teams~\cite{Debbiche2014:CI:Barrier}. Other barriers to CI include, setting up and maintaining a CI server~\cite{Hilton:fse2017:ci}, and changing development and testing practices within the team~\cite{Debbiche2014:CI:Barrier}. If a team chooses to adopt CI, then the team has to overcome these challenges, which can cost the team additional resources, for example effort and time.   

%%Continuous integration (CI) systems integrate code changes by automatically compiling, building, and executing test cases upon submission of code changes~\cite{Duvall:ci2007}. In recent years, usage of CI has become increasingly popular both for open source software (OSS) projects~\cite{hilton:ase2016:ci}~\cite{vasilescu2015quality}, as well as for proprietary projects~\cite{stahl:jss2017:ci:size}. Yet how CI influences and improves the software development process for proprietary software projects, remains unknown. With respect to CI adoption, practitioners can benefit from empirical case studies that address if adoption of CI significantly changes software development aspects such as collaboration amongst team members, resolution of bugs, and resolution of issues. These case studies can help practitioners to decide if CI is a good fit for their teams. Empirical evidence from the case studies, may also help address the skepticism that practitioners have about the benefits of CI adoption~\cite{Debbiche2014:CI:Barrier}.

%%%%%%%%%%%%%%%%%%%%%% BACKGROUND AND RELATED WORK 

%Practitioners often attribute Martin Fowler to first introduce the term continuous integration (CI). In a blog post from 2006~\cite{fowler:ci:2006}, Fowler stated continuous integration as the technique of ``where members of a team integrate their work frequently, usually each person integrates at least daily-leading to multiple integrations per day''.
% The CI process automatically builds integrated source code, and is considered as one of the fundamental pillars to implement continuous deployment~\cite{Humble:2010:CD} and DevOps~\cite{devops:software2016:elbort}.

%According to the Travis CI organization~\cite{travis:ci}, 932,977 projects use Travis CI for implementing CI. According to the State of Agile industry survey, 50\% of 3,880 participants have reported to use CI. 

%Authors from the State of DevOps report finds CI to be one of the indicators of `high performing IT organizations'.

%Furthermore, unlike traditional methodologies, software is delivered to customers rapidly, allowing the team to get customer feedback rapidly.

\subsection{Agile}
Agile methodology is highly collaborative and produces high quality solutions
in a cost effective and timely manner~\cite{moniruzzaman2013comparative}. Agile systems development methods emerged as a response to the inability of previous plan-driven approaches to handle rapidly changing environments~\cite{highsmith2002agile}. Williams and Cockburn~\cite{williams2003guest}
state that agile development is ``about feedback and change'', that agile methodologies
are developed to ``embrace, rather than reject, higher rates of change''. The frequent and regular feature delivery is achieved by team based approach and collaboration~\cite{coram2005impact}. Commits happening several times a day, without having problems in continuous integration is a good agile practice~\cite{vasilescu2014continuous, cusumano2007extreme}.

Deliver working software frequently, from a couple of weeks to a couple of months, with a preference for the shorter
timescale~\cite{williams2012agile, cusumano2007extreme}. Collective ownership of code is usually observed in agile~\cite{cusumano2007extreme}. On github, since, we have master branch which represents delivery of a software. If we have frequent deliveries, then we would be hoping to see commits happening at regular intervals. This would give a uniform distribution on the other hand as for the tradition method, we will see heavy commit every once in months. This kind of agile practice also promotes equal distribution of work done by each developer. We can extract such information by looking at the connectivity of social graph of developers. 

Agile practices allows to prioritize the requirements/issues, and aim to deliver them faster~\cite{moniruzzaman2013comparative}. This practice can be mapped to issues which are high and low priority problems in github and jira. And we want high priority problems to be solved first and faster than other low priority ones. Active customer involvement and  feedback denotes more discussions of a feature/issue~\cite{moniruzzaman2013comparative, sheffield2013factors}. This feature can be extracted from the issue and commit discussions.

Time, and cost  are all reduced when converting to agile from tradition methodology. Agile promises higher customer satisfaction, lower defect rates, and faster development times~\cite{moniruzzaman2013comparative}. The customer satisfaction and faster development could be mapped to lower the issues resolution time~\cite{mockus2002two}. And there should be large active discussions on these issues.

Agile developers take responsibility for producing cleaner code and to agreed standards~\cite{moniruzzaman2013comparative,sletholt2012we, williams2012agile, cusumano2007extreme}. By employing agile practices, problems with testing were less frequently reported than other traditional methods.~\cite{sletholt2012we}. Agile teams use practices like coding standards, peer
reviews, and pair programming to assure that the code they produce is technically solid~\cite{petersen2009comparison}. This feature could be mapped to how well commented the code is.

Agile development methods being more suitable for small teams than for larger team projects~\cite{dybaa2008empirical, gandomani2013obstacles, cusumano2007extreme}. Dybaa et al.~\cite{dybaa2008empirical} also reported agile (specifically, XP method) works best with experienced development teams. On the other hand Sheffield et al.~\cite{sheffield2013factors} reported that experience level of the team and project size do not explain agility. Small teams (12 people or less can be employed by getting rid of those developers who have committed very less commits. 

Reasons for adopting agile is to accelerate time to market, manage changing priorities, enhance software quality, reduce risk, reduce cost, simplify development process, improve team morale and enhance software maintainability~\cite{moniruzzaman2013comparative}. Team morale could be measured with sentiment analysis of their commit messages. Productivity of developers and project completion increases in agile methodology than traditional method~\cite{dybaa2008empirical}. Moniruzzaman et al.~\cite{moniruzzaman2013comparative} also showed that agile have more successful projects than traditional and that is the reason why many more companies are adapting towards the agile methodology. 

Agile practices benefit in terms of increased project success rate and user acceptance than traditional methods~\cite{moniruzzaman2013comparative}. The lower amount of bugs introduced which in turn can lower the cost and effort in a project. Customer is satisfied, team is satisfied tells a project is successful. The success can be measured by customer satisfaction and team satisfaction~\cite{sheffield2013factors}. Project popularity with stars, could be a quality measure as it denotes a well established project~\cite{tsay2014influence}.



Ilieva et al.~\cite{ilieva2004analyses} found 13\% fewer defects reported by the customer or by the quality assurance team in an XP
project than in a non-XP project. Changes produced by novice developers are more likely to introduce defects than those produced by subject matter experts~\cite{mcintosh2016empirical}. Users with lots of followers on github can be a matured developer~\cite{tsay2014influence}.
Pull requests are more likely to result in integration
testing failures than push commits.~\cite{vasilescu2014continuous} and bug location liklihood is more in such pull requests. The number of unique authors who have contributed less than 5\% of the changes could represent defective areas~\cite{mcintosh2016empirical}. Searching for defect-related keywords (error, bug, fix, defect, issue, mistake, incorrect, fault, and flaw etc.) in commit messages~\cite{vasilescu2014continuous}.


Vasilescu et al. [10] investigated quality and productivity issues when CI is used in open source projects, and reported that both productivity and quality increases upon adotion of CI tools

%%%%%% Added by Akond, June 26, 2017 
%%%%%% Related work on graph and network 
%%%%%% analysis in software engineering 

\subsection{Network-based Analysis in Software Engineering}
\label{sect:network-swe}

Researchers have extensively conducted network-based analysis
to identify network structure, communities, as well as to predict
defects. Bird et al.~\cite{Bird:SNA2006} mined email archives to identify which
network measures can be used to identify the social communication
nature of Apache HTTP Server project. The authors used three measures:
outdegree, in-degree and betweenness of a network, and observed strong relationships between email activity
and development activity. They also reported weak relationship between email activity
and document change activity.

Bird et al.~\cite{Bird:FSE2008} also mined email threads and used the concept of modularity to identify if community structures exist
in five open source software (OSS) projects namely, Apache, Ant, Python, Perl, and PostgreSQL.
They reported significant evidence of existing community structure amongst OSS projects. They also differentiated between
product and process-related emails, and observed an increase in modularity for product-related emails.

Hong et al.~\cite{Hong:ICSME2011} mined Mozilla bug reports to identify if the OSS network structure measures as similar to that of social network structures exhibited in social media websites such as Facebook and Twitter. They reported that unlike the social media sites, OSS projects do not exhibit power law distribution. They confirmed Bird et al.'s observations and reported that communities exhibit within a OSS project. Furthermore, they calculated in and out degree distributions and modularity, and reported that similar to social networks, OSS
project networks have strong communities and low degree of separation. They also reported that OSS project networks
have a smaller community size than that of social networks.

Shen and Monge~\cite{Shen:2011} mined Sourceforge projects to extract network-based metrics and identify the relationships
between developers. They observed that developers who are project leaders or experienced ina technology tend to
have lesser ties with other developers. Furthermore they observed  novice developers first tend to communicate with
fellow novice developers first, and gain experience and reputation. Once they
get experienced they tend to bond with other fellow experienced developers more.  

Zimmermann and Nagappan~\cite{Zimmermann:2007:SNA} investigated the value of network-based analysis
for predicting defective software binaries. They hypothesized that by extracting the dependencies
between binaries, a network can be formed. From the created network, network-based metrics such
as in-degree, betweenness, ego size can be extracted and used to predict defective binaries. They reported network-based
measures to be better than code complexity-based measures for predicting defective binaries. Their study was replicated by Premraj and Herzig
for three open source Java projects. Premraj and Herzig~\cite{premraj:herzig:esem2011} reported that code metrics are preferable than network-based
metrics for cross-project prediction and forward release prediction. They also reported that compared to network metrics
code metrics are easier to collect, and only eight code metrics might have comparable performance to 58 network-based metrics.
Similar views were echoed by Tosun et al.~\cite{Tosun:ESEM2009}. They also performed a replication of Zimmermann and Nagappan’s study for five small
scale projects. Tosun et al. reported that for small scale OSS projects, network-based metrics help in defect prediction, but offers no extra advantage over code-based metrics.

Bird et al.~\cite{Bird:FSE2011} conducted network analysis to investigate if developer contribution networks can be indicative of software quality. They
reported that count of minor contributors has a strong relationship with pre and post release software failures. They also reported that
metrics from contribution network is helpful in predicting pre release failures.

Zanetti et al.~\cite{Zanetti:ICSE2013} mined network-based metrics to classify bug report categories. They used two measures: centrality and connected components of a graph to predict the category of a bug report. They evaluated their methodology for for four OSS projects and observed
a F-measure of 0.67~0.92 for faulty models, in case of the four OSS projects.

Bhattacharya et al.~\cite{Bhattacharya:ICSE2012:GAP} hypothesized and provided evidence of how network-based measures can be used to predict effort and bug severity of
OSS projects. They used several network metrics: in degree, outdegree, node rank, diameter, assortativity, and clustering coefficient to detect
pivotal points of software development, and predict effort amount and bug severity. They reported that similar to biological networks,   software networks exhibit disassortative, where high degree nodes tend to connect with low degree nodes and vice versa.

Thung et al.~\cite{Thung:Github2013} mined Github data to identify influential projects and influential developers in a social coding platform e.g. Github.
They used node degree, pagerank, and shortest path, and provide a list of top five influential  projects  and influential developers
using a Github dataset of 100,00 software projects and 30,000 developers.

Lima et al.~\cite{lima:aaai:2014} mined Github data to identify follower, collaboration , and repository networks. They used network measures such as
assortativity, in-degree, out-degree, and clustering coefficient. They reported that the distributions of the number of contributors per project,
watchers per project, and followers per projects follow a power law-like shape. They also reported that very active users in Github do not have large amount of followers. They also observed that geographically close people tend to communicate and collaborate
more frequently than distant Github users.

Meneely et al.~\cite{Meneely:FSE2008} conducted an industrial case study to investigate if developer network analysis can be helpful in detecting software failures.They considered three metrics: degree, closeness, and betweenness. They reported that their network analysis-based prediction model can identify 58\% of the failures in 20\% of the files compared with the optimal prioritization that would have found 61\% in 20\% of the files. Their findings indicated that there is a significant relationship between file-based developer network metrics and failures.

In another paper, Meneely and Williams~\cite{Meneely:SNA:ICSE2011} reported that network-based measures represent the real-world scenario. In their paper they considered three network-based measures: developer network edges, developer network distances, and developer network centrality, and surveyed 124 practitioners. Their survey results indicated that developers networks are supported by developer perceptions, and
can be treated as a an approximation of the real world complex activity of developers.   

The above-mentioned studies indicate that in software projects network-based measures such as degree calculation, assortativity
can be helpful in identifying project characteristics. Network-based measures such as modularity can be helpful in detecting
latent social strictures that exist for software projects. Furthermore, network measures are also related to software reliability and quality: we can use network-based metrics to predict defects and failures.  

% Recently, the influence and adoption of CI has gained interest amongst researchers. Hilton et al.~\cite{hilton:ase2016:ci} have investigated adoption rate of CI in OSS Github projects. Other researchers have investigated if CI influences bug resolution~\cite{vasilescu2015quality}, commit patterns~\cite{Zhao:ASE17:CI}, and issue resolution~\cite{Zhao:ASE17:CI} for OSS %Github projects. 
 
%Shahin et al.~\cite{shahin:access2017:ci} investigated which practices should be considered while adopting CI, and provided four recommendations: reducing build and test time, increasing awareness on build results, supporting automated continuous testing, and defect detection.

%Stahl et al.~\cite{stahl:jss2017:ci:size} surveyed practitioners and mined software data, and reported that continuity of continuous integration and organization size is correlated. In another study, 

%Rahman et al.~\cite{Rahman:RCOSE17} investigated which diffusion of innovation (DOI) factors influence CI tools, and reported four factors to influence adoption of CI tools: relative advantages, compatibility, complexity, and education. Hilton et al.~\cite{Hilton:fse2017:ci} surveyed industry practitioners and identified three trade-offs to adopt CI: assurance, flexibility, and security.

%Beller et al.~\cite{beller:msr2017} synthesized the nature of build and testing attributes exhibited amongst open source projects that use CI. Storm~\cite{storm:ci:saner2008} used the concept of backtracking to resolve build failures that happen in a CI system. Rausch et al.~\cite{rausch:msr2017:ci} investigated build failures from 14 Java-based systems and characterized 14 error categories. They also observed that process metrics have relatively more influence on CI build failures. Zampetti et al.~\cite{zampetti:msr2017:ci} investigated the use of static analysis tools in a CI-based workflow, and reported that the main reason builds fail is due to not maintaining coding standards.


%%%%%%%%%%%%%%%%%%%%%%%%% MOTIVATION %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \section{Motivating Examples}
% \label{motive}
% In this section we provide two hypothetical examples that motivate our empirical study. The names presented in the examples are imaginary. 

% Bob is a manager of software development team, which develops desktop and mobile applications. To facilitate the development process on a wide range of platforms, the team uses a wide range of tools including enterprise mobile development kits, enterprise IDEs, and a CI tool. Recently, management has advised Bob to cut costs by identifying tools that does not contribute to collaboration and bug resolution. Bob wants to make an informed decision, but unfortunately, the team does not have a data scientist who can help him by mining and analyzing their existing software repositories. To make an informed decision, Bob now has to explore industry and research articles that have investigated if introduction of CI impacts resolution of bugs and collaboration. 

% Alice is a new member of a software development team. Alice's team develops and maintains open source and proprietary projects, but the team does not use CI. Alice has used CI as part of fulfilling her graduate course requirements, and wants to introduce CI to the team. She introduces the idea of adopting CI in a team meeting, and observes skepticism from her colleagues. Her colleagues of CI's impact on bug and issue resolution, and asks for concrete empirical evidence both in the OSS and the proprietary domain. Alice acknowledges the need of empirical evidence, and starts browsing industry-focused white papers, as well as research papers that provided sufficient empirical evidence on how CI can impact issue and bug resolution for OSS and proprietary projects.      

% \textit{\textbf{The above-mentioned examples highlight the information needs for making management decisions for CI adoption}}. Our paper can helpful in both of the above-mentioned example scenarios. We systematically investigate the impact of CI on collaboration, bug resolution, and issue resolution, with statistical rigor.  

%%%%%%%%%%%%%%%%%%%%% METHODOLOGY %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\item{\textit{Start Date}: The project must start on or after January, 2011. Projects older than 2011 can skew the overall calculation of metrics obtained before and after adopting a CI tool, and should be excluded. Popular CI tools such as Travis CI was first introduced in 2011, and our assumption is that by excluding projects that started before 2011, we can reduce skewness. Our approach is similar to Hilton et al.~\cite{hilton2016usage}.}

We select edge count because in collaboration graphs, edges correspond to collaboration, more edges imply programmers collaborating more with each other on a project. We select in-degree because, similar to edges, in-degree also correspond to collaboration between the programmers. The higher the average and median in-degree, the higher connection is between the nodes~\cite{sna:degree:mahadevan:sigcomm2007}~\cite{Bhattacharya:ICSE2012:GAP}, indicating more collaboration between the programmers.   

Projects can vary in node size, and needs to be accounted for~\cite{Hong:ICSME2011}. Similar to Hong et al.~\cite{Hong:ICSME2011} and Bird et al.~\cite{Bird:SNA2006}, we normalize these three measures by the count of nodes. We use Equation~\ref{equ:ec}, and~\ref{equ:mid}, respectively to normalize edge count, and median in-degree.    

\begin{equation}
EdgeCount (EC) = \frac{\text{total count of edges}}{\text{total count of nodes}}\label{equ:ec}
\end{equation}

\begin{equation}
Median In-Degree (MID) = \frac{\text{median in-degree}}{\text{total count of nodes}}\label{equ:mid}
\end{equation}

%\begin{equation}
%Average In-Degree (AID) = \frac{\text{average in-degree}}{\text{total count of nodes}}\label{equ:aid}
%\end{equation}

Finally, we aggregate the graph metrics for each project, and normalize with the respect to time. We use Equations~\ref{equ:nec},and ~\ref{equ:nmid}, respectively, to calculate `Normalized Edge Count', and `Normalized Median In-Degree'. 

\begin{equation}
Normalized Edge Count (NEC) =  \dfrac{\sum_{i=1}^{M}EC(i)}{M}\label{equ:nec}
\end{equation}

\begin{equation}
Normalized Median In-Degree (NMID) =  \dfrac{\sum_{i=1}^{M}MID(i)}{M}\label{equ:nmid}
\end{equation}

%\begin{equation}
%Normalized Average In-Degree (NAID) =  \dfrac{\sum_{i=1}^{M}MID(i)}{M}\label{equ:naid}
%\end{equation}

Similar to issues stated in ~Section~\ref{meth:rq1}, and bugs stated in Section~\ref{meth:rq2}, we compute $NEC$, and $NMID$, for all projects, before and after adoption of CI. We apply statistical tests, described in Section~\ref{meth:stat}, to determine if CI has an impact on collaboration.

%Cliffs cutoff: https://www.bibsonomy.org/bibtex/216a5c27e770147e5796719fc6b68547d/kweiand and https://www.rdocumentation.org/packages/effsize/versions/0.6.4/topics/cliff.delta

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%RESULTS%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Sanity check & \multicolumn{2}{c|}{Discarded project count}                     \\ \cline{2-3} 
%                                           & \multicolumn{1}{l|}{Proprietary} & \multicolumn{1}{l|}{OSS} %\\ \hline

%Upon completion of Filter-2 we are left with 123 proprietary and 150 OSS projects.
%Upon completion of Filter-1 we are left with 171 proprietary and 661 OSS projects.

%Sanity check & \multicolumn{2}{c|}{Discarded project count}                     \\ \cline{2-3} 
%                                         & \multicolumn{1}{l|}{Proprietary} & \multicolumn{1}{l|}{OSS} \\

%Time Period         & Jan, 2014 - Jul, 2017 & Jan, 2014 - Jun, 2017 \\

\begin{figure*}
\subfloat[]{
 \includegraphics[width=0.23\textwidth]{plots/OSS_NORM_OPEN_ISS_RATIO.png}
 \label{fig:res:noi:oss}
}
\subfloat[]{
 \includegraphics[width=0.23\textwidth]{plots/PROP_NORM_OPEN_ISS_RATIO.png}
 \label{fig:res:noi:pro}
}
\subfloat[]{
 \includegraphics[width=0.23\textwidth]{plots/OSS_NORM_CLOSE_ISS_RATIO.png}
 \label{fig:res:nci:oss}
}
\subfloat[]{
 \includegraphics[width=0.23\textwidth]{plots/PROP_NORM_CLOSE_ISS_RATIO.png}
 \label{fig:res:nci:pro}
}
\caption{Normalized open and closed issues for open source and proprietary projects. Figure~\ref{fig:res:noi:oss} presents the normalized count of open issues in open source projects. Figure~\ref{fig:res:noi:pro} presents the normalized count of open issues in proprietary projects. Figure~\ref{fig:res:nci:oss} presents the normalized count of closed issues in open source projects. Figure~\ref{fig:res:nci:pro} presents the normalized count of closed issues in proprietary projects.} 
\label{fig:res:rq1} 
\end{figure*}

\begin{table}
\caption{Influence of CI on Issue Resolution}
\centering
\small{
\begin{tabular}{ |c|c|c|c|c| } 
\hline
            & NOI             &                & NCI             &                 \\ 
\hline
Measure     & OSS             & Prop.          & OSS             & Prop.           \\ 
\hline
Mean        & (A:0.5, B:0.2)  & (A:0.1, B:0.0) & (A:0.3, B:0.1)  & (A:0.1, B:0.0)  \\ 
Median      & (A:0.5, B:0.1)  & (A:0.1, B:0.0) & (A:0.3, B:0.0)  & (A:0.0, B:0.0)  \\ 
p-value     & $< 0.001$       & $< 0.001$      & $< 0.001$       & $< 0.001$       \\ 
Cliffs      & 0.8             & 0.3            & 0.7             & 0.3             \\ 
SK (Ranks)  & (A:1, B:3)      & (A:1, B:3)     & (A:2, B:4)      & (A:2, B:4)      \\ 
\hline
\end{tabular}
}
\label{table:rq1}
\end{table}

%: we observe that for OSS Github projects, number of closed issues increases after adoption of CI

\begin{figure*}
\subfloat[]{
 \includegraphics[width=0.23\textwidth]{plots/OSS_NORM_OPEN_BUG_RATIO.png}
 \label{fig:res:nob:oss}
}
\subfloat[]{
 \includegraphics[width=0.23\textwidth]{plots/PROP_NORM_OPEN_BUG_RATIO.png}
 \label{fig:res:nob:pro}
}
\subfloat[]{
 \includegraphics[width=0.23\textwidth]{plots/OSS_NORM_CLOSE_BUG_RATIO.png}
 \label{fig:res:ncb:oss}
}
\subfloat[]{
 \includegraphics[width=0.23\textwidth]{plots/PROP_NORM_CLOSE_BUG_RATIO.png}
 \label{fig:res:ncb:pro}
}
\caption{Normalized open and closed bugs for open source and proprietary projects. Figure~\ref{fig:res:nob:oss} presents the normalized count of open bugs in open source projects. Figure~\ref{fig:res:nob:pro} presents the normalized count of open bugs in proprietary projects. Figure~\ref{fig:res:ncb:oss} presents the normalized count of closed bugs in open source projects. Figure~\ref{fig:res:ncb:pro} presents the normalized count of closed bugs in proprietary projects.} 
\label{fig:res:rq2} 
\end{figure*}

\begin{table}
\caption{Influence of CI on Bug Resolution}
\centering
\small{
\begin{tabular}{ |c|c|c|c|c| } 
\hline
            & NOB             &                & NCB                            & \\ 
\hline
Measure     & OSS             & Prop.          & OSS             & Prop.           \\ 
\hline
Mean        & (A:0.3, B:0.1)  & (A:0.0, B:0.0) & (A:0.2, B:0.0)  & (A:0.0, B:0.0)  \\ 
Median      & (A:0.3, B:0.0)  & (A:0.0, B:0.0) & (A:0.1, B:0.0)  & (A:0.0, B:0.0)  \\ 
p-value     & $< 0.001$       & 0.1            & $< 0.001$       & 0.01            \\ 
Cliffs      & 0.5             & 0.0            & 0.5             & 0.1             \\ 
SK (Ranks)  & (A:1, B:3)      & (A:1, B:2)     & (A:2, B:4)      & (A:1, B:2)      \\ 
\hline
\end{tabular}
}
\label{table:rq2}
\end{table}

\subfloat[]{
 \includegraphics[width=0.32\textwidth]{plots/PROP_NORM_ADEG.png}
 \label{fig:res:naid:pro}
}

\begin{table*}
\caption{Influence of CI on Collaboration}
\centering
\small{
\begin{tabular}{ |c|c|c|c|c|c|c| } 
\hline
            & NEC             &                & NMID            &                  & NAID            &         \\ 
\hline
Measure     & OSS             & Prop.          & OSS             & Prop.            & OSS             & Prop.   \\ 
\hline
Mean        & (A:0.5, B:0.4)  & (A:0.3, B:0.3) & (A:0.1, B:0.0)  & (A:0.1, B:0.0)   & (A:0.1, B:0.0)  & (A:0.1, B:0.0) \\ 
p-value     & 0.07            & 0.08           & $< 0.001$       & $< 0.001$        & $< 0.001$       & 0.001      \\ 
Cliffs      & 0.1             & 0.2            & 0.2             & 0.2              & 0.2             & 0.2       \\ 
\hline
\end{tabular}
}
\label{table:rq3}
\end{table*}

\subsection{Explanation}

\begin{figure}
\subfloat[]{
 \includegraphics[width=0.25\textwidth]{plots/OSS_NORM_NCNT.pdf}
 \label{fig:res:nnc:oss}
}
\subfloat[]{
 \includegraphics[width=0.25\textwidth]{plots/PROP_NORM_NCNT.pdf}
 \label{fig:res:nnc:pro}
}
\caption{Active programmer count for OSS and proprietary projects, before and after adoption of CI. Figures~\ref{fig:res:nnc:oss}~\ref{fig:res:nnc:pro} respectively presents the normalized count of programmers before and after adoption of CI, for OSS and proprietary projects.} 
\label{fig:res:rq3:nnc} 
\end{figure}

\begin{table}
\caption{Count of Programmers Before and After Adoption of CI }
\centering
\small{
\begin{tabular}{ |c|c|c| } 
\hline
Measure     & OSS       & Prop.           \\ 
\hline
p-value     & 0.23       & 0.86            \\ 
Cliffs      & 0.04       & 0.08             \\ 
\hline
\end{tabular}
}
\label{table:node:count:res}
\end{table}

\begin{figure*}
\subfloat[]{
 \includegraphics[width=0.5\textwidth]{plots/OSS_NORM_SELF_EDGE.pdf}
 \label{fig:res:nse:oss}
}
\subfloat[]{
 \includegraphics[width=0.5\textwidth]{plots/PROP_NORM_SELF_EDGE.pdf}
 \label{fig:res:nse:pro}
}
\caption{Self modification count for OSS and proprietary projects, before and after adoption of CI. Figures~\ref{fig:res:nse:oss}~\ref{fig:res:nse:pro} respectively presents the normalized count of self modifications made by programmers before and after adoption of CI, for OSS and proprietary projects.} 
\label{fig:res:rq3:nse} 
\end{figure*}


\begin{table}
\caption{Influence of CI on Self Modifications}
\centering
\small{
\begin{tabular}{ |c|c|c| } 
\hline
Measure     & OSS       & Prop.           \\ 
\hline
p-value     & 0.48       & 0.74            \\ 
Cliffs      & 0.00       & 0.05             \\ 
\hline
\end{tabular}
}
\label{table:self:edge:res}
\end{table}

\subsection{RQ3: How does usage of continuous integration influence collaboration in open source and proprietary projects?}
\label{res:rq3}


\begin{figure*}
\subfloat[]{
 \includegraphics[width=0.25\textwidth]{plots/OSS_NORM_ECNT.pdf}
 \label{fig:res:nec:oss}
}
\subfloat[]{
 \includegraphics[width=0.25\textwidth]{plots/PROP_NORM_ECNT.pdf}
 \label{fig:res:nec:pro}
}
\subfloat[]{
 \includegraphics[width=0.25\textwidth]{plots/OSS_NORM_MDEG.pdf}
 \label{fig:res:nmid:oss}
}
\subfloat[]{
 \includegraphics[width=0.25\textwidth]{plots/PROP_NORM_MDEG.pdf}
 \label{fig:res:nmid:pro}
}
\caption{Influence of CI on collaboration metrics. Figure~\ref{fig:res:nec:oss} and Figure~\ref{fig:res:nec:pro} respectively presents the edge count for OSS and proprietary projects. Figure~\ref{fig:res:nmid:oss} and Figure~\ref{fig:res:nmid:pro} respectively presents the median in-degree for OSS and proprietary projects.} 
\label{fig:res:rq3} 
\end{figure*}


As described in Section~\ref{meth:rq3}, we report the normalized edge count and the normalized median in-degree for OSS and proprietary projects to answer RQ3. We report the summary statistics in Table~\ref{table:rq3}, and the present the box-plots in Figure~\ref{fig:res:rq3}. According to Table~\ref{table:rq3}, for edge count the difference before and after adoption of CI is not significant. On the other hand, for both OSS and proprietary and projects, the median in-degree significantly increases after adoption of CI. The effect size for OSS and proprietary projects is 0.2, which is small according to Romano et al.~\cite{Romano:CliffsCutoff2006}. Based on Cliffs Delta, we also observe that the influence of CI is not as large as closed issues or closed bugs for OSS projects, as reported in Section~\ref{res:rq1} and Section~\ref{res:rq2}, respectively.  

\vspace{1mm} %1mm vertical space
%%%Lesson-3 in a box 
\fbox{\begin{minipage}{25em}
\small{\textbf{\textit{\underline{Lesson-3}: CI influences collaboration for OSS and proprietary projects. After adoption of CI collaboration between programmers significantly increases.}}}
\end{minipage}}

\begin{table}
\caption{Influence of CI on Collaboration}
\centering
\small{
\begin{tabular}{ |c|c|c|c|c| } 
\hline
            & \textbf{Edge Count} &                & \textbf{Median In-degree} &                  \\ 
\hline
Measure     & OSS                 & Prop.          & OSS                       & Prop.            \\ 
\hline
p-value     & 0.07                & 0.08           & $< 0.001$                 & $< 0.001$        \\ 
Cliffs      & 0.1                 & 0.2            & 0.2                       & 0.2              \\ 
\hline
\end{tabular}
}
\label{table:rq3}
\end{table}

% The median $NCC$ is respectively, 2.2, and 0.9, after and before adoption of CI for OSS, which indicates that after adoption of CI, programmers make 2.4 times more commits than that of before adopting CI. Based on median $NCC$, the commit count for proprietary projects decreases from 1.1 to 0.7, after adoption of CI.

%Our answers to RQ4 can provide further evidence to this explanation.  
%Future research can take this finding into account, and investigate even further. 
%In Table~\ref{table:rq3}, the `delta' metric is represented in the $\Delta$ row. The `delta' measures for which we observe no significant difference is highlighted in grey.  

% According to Table~\ref{table:rq4}, after CI adoption programmers make significantly more commits in OSS projects, but not in our set of proprietary projects.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%DISCUSSION 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%As discussed in Section~\ref{results}, the influence of CI is observable more for OSS projects, compared to proprietary projects.

%An automated process of data mining and data analysis can help practitioners to perform continuous analytics.
%Existing APIs such as the Github API, Jira API, and Travis API, can be helpful in this regard. 
%By mining software repositories, and applying data analytics we have observed that CI has an influence on issue and bug resolution for OSS projects, but not for proprietary projects. Our findings indicate that data analytics and data mining can be an integral part of their software development process. We make the following recommendations: 
%\begin{itemize}[leftmargin=*]
%\item{\textbf{Mining software repositories:} Software practitioners can mine features such as bugs, commits, and issues form version control meta-data, and use these features to make informed decisions. Existing APIs such as the Github API, Jira API, and Travis API, can be helpful in this regard. }
%\item{\textbf{Continuous analytics for decision making:}  }
%\end{itemize}

%\textbf{Differences in Open Source and Proprietary Projects:} Our answers to RQ1, RQ2, and RQ4 state that the impact of CI is different for OSS and proprietary projects. The difference in our findings can be attributed to the differences in software development that exists between OSS and proprietary projects~\cite{Paulson:TSE2004}~\cite{Robinson:esem2010:prop:oss}. Our findings indicate that CI may not fulfill practitioners' needs in the same manner for OSS and proprietary projects. Both researchers and practitioners can benefit form our findings. One implication of our findings for practitioners is that with respect to tool adoption, practitioners cannot rely only on the experience of other practitioners. With respect to tool adoption, practitioners follow the `diffusion of innovation' rule, which states that practitioners prefer to learn from other practitioners who have already adopted the tool of interest~\cite{akond:agile2015:cd}~\cite{rogers2010diffusion}. Learning from other practitioners can be a starting point, but practitioners also need to (i) consider their teams' development context factors, and (ii) assess to what extent the prior practitioners' experiences hold.    

%In prior work, researchers~\cite{vasilescu2015quality}~\cite{Zhao:ASE17:CI}~\cite{hilton:ase2016:ci} have investigated the impact of CI using OSS projects, but not for proprietary projects. Our findings suggest that only investigating OSS projects to understand a phenomenon might be be in-comprehensive. We acknowledge that collecting, mining, and reporting on proprietary datasets is non-trivial. We argue for better collaboration between academic researchers and industry practitioners. 


%We further illustrate our findings using Figure~\ref{fig:disc:explain}. Inspired by prior work~\cite{madachy2007software} on software process dynamics, we provide two explanatory models in Figure~\ref{fig:disc:explain} that explains how commit frequency is related to bug and issue resolution. Figure~\ref{fig:disc:explain:issue} provides an explanatory model, where `Open Issues' are converted into `Closed Issues'. The conversion process is dependent on a control variable called `Commit Frequency'; if commit frequency is higher then more open issues will be converted to closed issues. The control variable is influenced by the variable `Continuous integration': presence of `Continuous integration' in OSS influences `Commit frequency'. As shown in Figure~\ref{fig:disc:explain:bug}, our explanatory model for bug resolution is similar to that of issues. The conversion of `Open Bugs' to `Closed Bugs' is dependent on the control variable `Commit Frequency'. Our datasets and empirical analysis cannot offer exact numeric relations for the two explanatory models, but these explanatory models might support a fruitful line of future research. 

%Based on our findings we recommend practitioners to commit frequently to utilize CI tools properly. 

%Researchers~\cite{Passos:2013:ESEM:Belief} have reported that practitioners' perceptions can impact the adoption of a technology.
%Future research can investigate and quantify the relationship between rapid feedback provided by CI, and software quality and productivity. 

%\begin{figure}
%\subfloat[]{
% \includegraphics[width=0.22\textwidth]{plots/explain-issue-res.pdf}
% \label{fig:disc:explain:issue}
%}
%\subfloat[]{
% \includegraphics[width=0.22\textwidth]{plots/explain-bug-res.pdf}
% \label{fig:disc:explain:bug}
%}
%\caption{Explanatory models for bug and issue resolution. Figure~\ref{fig:disc:explain:bug} and Figure~\ref{fig:disc:explain:issue} respectively, explains how %commit frequency is related to bug and issue resolution.} 
%\label{fig:disc:explain} 
%\end{figure}

%The name `cargo cult' derives from the belief which began among Melanesians since the 1900s where various ritualistic acts such as the building of an airplane runway will result in the appearance of  Western goods (i.e., `cargo'), via Western airplanes.   
%One possible   
%Cargo cults  arise when one culture meets a  more technologically advanced societies~\cite{wiki:cargocult}.
%The concern of this paper is that proprietary projects suffer from a cargo cult mentality with respect to OSS tools.
%As a result, proprietary project owners, are not reaping the benefits of CI adoption, even they have adopted CI tools. 


%\textbf{Future Research on CI:} We observe the opportunity for further research in CI through software analytics. Future studies can confirm/refute our findings with a bigger set of projects, collected from multiple organizations. Previously, researchers~\cite{vasilescu2015quality}~\cite{Zhao:ASE17:CI}~\cite{hilton:ase2016:ci} have investigated the influence of CI using OSS projects, but not for proprietary projects. Our findings suggest that only investigating OSS projects to understand the CI process might be be in-comprehensive. With respect to CI, we encourage researchers to investigate projects both from the OSS and proprietary domain. We acknowledge that collecting, proprietary datasets is non-trivial. We argue for better collaboration between academicians and practitioners. 


%%%%%% DISCUSSION 

%Based on the analysis of OSS GitHub projects, Hilton et al.~\cite{hilton:ase2016:ci} strongly advocated for CI adoption stating ``developers should consider CI as a best practice and should use it widely as possible''.

% The fact that unlike OSS projects, the benefits of CI is not applicable for our set of proprietary projects deserves explanation
% We restrain ourselves from making similar recommendations for proprietary projects, as we do not observe CI to have influence on two attributes of software development for proprietary projects.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%THREATS 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%In Github, a bug might not be marked in an issue but in commits. We plan to investigate how bugs can inferred from commits, and update our findings accordingly. 
%We have used file modification history to construct graphs and assess the collaboration level of the project. We acknowledge that relying on one concept might not comprehensive. Our analysis is conducted per month, which might not fine-grained. In future, we plan to investigate if our findings hold for other granularity of time unit such as per week, or per-year. 


\section{Limitations}
\label{limitation}
We discuss the limitations of our research study as following: 

\begin{itemize}
\item{\textbf{Generalizability}: We conducted our empirical study using open source projects hosted on Github, and proprietary projects belonging to IBM. We acknowledge that our selected set of projects are not comprehensive. We plan to add more projects from other data sources such as SourceForge, and from other companies. }

\item{\textbf{CI}: In our paper we have adopted a heuristic-driven approach to detect use of CI in a project. We acknowledge that our heuristic is limited tot he three CI tools, and we plan to improve our heuristics by exploring the possibility to add more CI tools. }

\item{\textbf{Bug Resolution}: We have relied on issues marked as a `bug' to count bugs and bug resolution time. In Github, a bug might not be marked in an issue but in commits. We plan to investigate how bugs can inferred from commits, and update our findings accordingly.  }

\item{\textbf{Collaboration Graph}: We have used one concept (modification of files) to construct graphs and assess the collaboration level of the project. We acknowledge that relying on one concept might not comprehensive. }

\item{\textbf{Granularity}: Our analysis is conducted per month, which might not fine-grained. In future, we plan to investigate if our findings hold for other granularity of time unit such as per week, or per-year. }

\end{itemize}


%%%%%%%%%%%%%%% ACK
%Special thanks to Bo Zhang, Donald Cronin, Jamie Jennings, and Joe Hughes for their valuable feedback.   

==> menzies.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%% MSR INTRO %%%%%%%%%%%%%%%%%%%%

Numerous writers   in the industrial press (see S1.1)
caution that   some organizations pretend to ``do agile'' without
actually ``being agile'';
i.e. without actually adopting all the agile pratices that make agile
tools most useful.
While their cautions seem sensible, for the most part, they are made
with little to no
empirical support. Accordingly, this paper paper checks empirically
for two effects:
\bi
\item  Are some projects ``doing agile'' without ``being agile''?
\item  Are those projects   suffer from any detrimental effects?
\ei
To focus this research, we explore
 the agile practice of continuous intergration (CI). CI systems
integrate code changes by automatically
compiling, building, and executing test cases upon submission of
code changes. In recent years, usage of CI tools has become increasingly
popular both for open source software (OSS) projects [18] [38], as
well as for proprietary projects [
37
].
This paper compares the affect of adopting CI for open source software
(OSS) projects [18] [38]
using data mined from 661 OSS projects and
171 proprietary projects from a cloud-programming development
environment hosted at Research Triangle, Raleigh, North Carolina.

We find much evidence that many of those proprietary projects  are
``doing agile''
(i.e. they are adopting CI tools) without actually ``being agile''. We
show this by
answering   four research questions:

RQ1: How does adoption of continuous integration influence
issue resolution?
Significantly more issues are resolved after
adoption of CI for OSS projects, but not for proprietary projects.
RQ2: How does adoption of continuous integration influence
bug resolution?
Unlike proprietary projects, significantly more
bugs are resolved after adoption of CI within OSS projects.
RQ3: How does adoption of continuous integration influence
collaboration amongst team members?
After adopting CI, col-
laboration significantly increases for both, OSS and proprietary
projects. The increase in collaboration is more observable for OSS
projects, than proprietary projects.
RQ4: Does adoption of continuous integration influence com-
mit patterns?
Commit frequency and sizes significantly increases
for OSS projects after CI adoption, but not for proprietary projects

Based on the above, we advise:
\begin{quote}
{\em Do not use the tools from another community without also
adopting the practices of that community.}
\end{quote}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%% ABSTRACT %%%%%%%%%%%%%%%%%%%%%
%Recently there has been widespread adoption of open source software (OSS) development tools and practices by in-house proprietary projects. Do those proprietary projects reap the benefits of those tools--specifically, continuous integration (CI) tools? 
%those tools--specifically, continuous integration (CI) tools? how CI influences the software development process for both, open source software (OSS) and proprietary projects
%and more collaboration between team members
%Why is this so? We argue that mere tool use is not enough to improve software development. Tools carry within them the cultural assumptions of  their creators. Adopting a tool, without also adopting the culture of the tool creators, can be a mistake. Much of the benefit of CI arises from increased interaction between team members when new code is committed. Our proprietary projects, that commit less often, miss that benefit.
%Tools carry within them the cultural assumptions of  their creators. Adopting a tool, without also adopting the culture of the tool creators, can be a mistake.
%increased interaction between team members when new code is committed
%More generally, when considering new tools, organizations are advised to reflect much more not only on a tool's capabilities, but also on the culture of the community that created those tools.

%%%%%%%%%%%%%%%%%%%%%%%%% INTRO %%%%%%%%%%%%%%%%%%%%%%%%
%of the open source software (OSS) community
%When adopting tools,  it may also be necessary to adopt the culture where those tools were developed.
%our industrial collaborators at Research Triangle Park, North Carolina
%Practitioners perceive adoption and usage of CI help them in catching bugs earlier, make integration of software changes easier, and make frequent releases of software product~\cite{fowler:ci:2006}~\cite{hilton:ase2016:ci}.

%This paper is about the `cult' of continuous integration (CI) and what goes wrong when preparatory software development projects adopt the tools, but not the best practices. A software process anti-pattern will be reported where proprietary projects suffer the cost of process change without reaping the benefits of those tools. This pattern is not rare: we have observed in 171 proprietary software development projects. 
%tend to commit/review less often than open source projects, do not achieve those benefits
%open source (faster bug resolution, issues closed more frequently, more collaboration between team member)

% Our empirical study reveals the following findings: 
% \begin{itemize}[leftmargin=*]
% \item{Adoption of CI has an influence on closed issues for OSS projects, but not for proprietary projects. For OSS projects, significantly more issues are closed after adoption of CI.}
% \item{Unlike proprietary projects, significantly more bugs are resolved after adoption of CI.}
% \item{Collaboration significantly increases after adoption of CI, but much more for  OSS than proprietary projects.}
% \item{After adoption of CI, commit frequency and sizes significantly increases for OSS projects, but not for proprietary projects.}
% \end{itemize}
% Based on our findings we recommend: 
% \begin{itemize}[leftmargin=*]
% \item{With respect to CI adoption, practitioners should consider their team's development context.}
% \item{After adoption of CI, practitioners should investigate if CI satisfies practitioners' needs by applying software analytics.}
% \end{itemize}

%Our results are very much in alignment with Brooks' warnings. Even in the best case reported below (from OSS projects), the improvements due to CI are only a XXXX double or tripling of XXX; i.e. far less than the order of magnitude improvements promised by mythical silver bullet technology. 

%\item
%Strongly recommend CI for OSS.

%That said, the gains  from CI are large enough to make us:

%\begin{itemize}
%\item
%Strongly recommend that proprietary organize themselves differently to achieve the benefits of CI.
%\end{itemize}

%we provide two motivational examples in Section.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% RELATED WORK AND BACKGROUND  
%All the above work focuses on OSS projects. 

\subsection{Cargo Cults and Silver Bullets}
\label{bg:cult:bullet}
One way to summarize this  paper is to say that proprietary projects are mimicking OSS practices but are missing an essential part of those practices.
That is, the managers of proprietary projects are treating OSS like some sort of `cargo cult'. Cargo cults  arise when one culture
meets a  more technologically advanced societies~\cite{wiki:cargocult}. Lindstrorm~\cite{Lindstrom93} characterizes such cargo cults as the mimicry of part of another culture, but missing an essential part of those practices. The name `cargo cult' derives from the belief which began among Melanesians since the 1900s where various ritualistic acts such as the building of an airplane runway will result in the appearance of  Western goods (i.e., `cargo'), via Western airplanes. For example, after World War II in Vanuatu, cargo cult members worshiped mythical  Americans named `John Frum' or `Tom Navy' who brought cargo to their island during World War II and who would, it was believed,  will  provide cargo to them in the future. Cargo cults persist, even to this day~\cite{dimeo10}. The concern of this paper is that proprietary projects suffer from a cargo cult mentality with respect to OSS tools. 

Researchers~\cite{Spinellis07} in prior work warned against `silver bullets' in software engineering. In Brooks' 1986 paper `No Silver Bullet-- Essence and Accident in Software Engineering'~\cite{Brooks87}, he warns against hyping a technology as the `silver bullet' that will automatically kills the werewolves which bedevil software engineering.
 
\begin{quote}
{\em ``There is no single development, in either technology or management technique, which by itself promises even one order of magnitude improvement within a decade in productivity, in reliability, in simplicity.''~\cite{Brooks87}}
\end{quote}

\section{Background}
We first briefly describe the concepts of `cargo' and `silver bullets' in Section~\ref{bg:cult:bullet}. Next we provide background on CI and discuss related work in Section~\ref{bg-ci}.

\subsection{Cargo Cults and Silver Bullets}
\label{bg:cult:bullet}
One way to summarize this  paper is to say that proprietary projects are mimicking OSS practices but are missing an essential part of those practices.
That is, the managers of proprietary projects are treating OSS like some sort of `cargo cult'. Cargo cults  arise when one culture
meets a  more technologically advanced societies~\cite{wiki:cargocult}. Lindstrorm~\cite{Lindstrom93} characterizes such cargo cults as the mimicry of part of another culture, but missing an essential part of those practices. The name `cargo cult' derives from the belief which began among Melanesians since the 1900s where various ritualistic acts such as the building of an airplane runway will result in the appearance of  Western goods (i.e., `cargo'), via Western airplanes. For example, after World War II in Vanuatu, cargo cult members worshiped mythical  Americans named `John Frum' or `Tom Navy' who brought cargo to their island during World War II and who would, it was believed,  will  provide cargo to them in the future. Cargo cults persist, even to this day~\cite{dimeo10}. The concern of this paper is that proprietary projects suffer from a cargo cult mentality with respect to OSS tools. 

Motivated by Brooks, we investigate if CI positively impact four aspects of software development, namely, bug resolution, collaboration, issue resolution, and commit patterns. If Brooks observations hold, then we will observe CI to not have an impact on bug resolution, collaboration, and issue resolution.  



%%%%%%%%%%%%%%%%%%%%%%CONCLUSION 
%To be clear, when we say ``CI tools have little to no benefit on proprietary projects'', we should say ``no benefit {\em as detected by the measurements of this study}'' i.e. faster bug resolution, issues closed more frequently, more collaboration between team member. There may well be other benefits of introducing CI  that are not captured by our measurements. For example,  management might  adopt CI tools to recruit more next generation programmers. 
